Learning Population-level Shape Statistics and Anatomy Segmentation From Images: A Joint Deep Learning Model

Statistical shape modeling is an essential tool for the quantitative analysis of anatomical populations. Point distribution models (PDMs) represent the anatomical surface via a dense set of correspondences, an intuitive and easy-to-use shape representation for subsequent applications. These correspondences are exhibited in two coordinate spaces: the local coordinates describing the geometrical features of each individual anatomical surface and the world coordinates representing the population-level statistical shape information after removing global alignment differences across samples in the given cohort. We propose a deep-learning-based framework that simultaneously learns these two coordinate spaces directly from the volumetric images. The proposed joint model serves a dual purpose; the world correspondences can directly be used for shape analysis applications, circumventing the heavy pre-processing and segmentation involved in traditional PDM models. Additionally, the local correspondences can be used for anatomy segmentation. We demonstrate the efficacy of this joint model for both shape modeling applications on two datasets and its utility in inferring the anatomical surface.

==> introduction_old.tex <==

\section{Introduction}

Shape representation is an important step for statistical shape analysis of anatomical shape population; it involves representing the surface of the anatomy in a consistent manner. Furthermore, a shape representation allows for subsequent statistics for any downstream application utilizing shape information. Particle distribution models (PDM) \cite{greneder}, represents the shapes via a set of dense \emph{correspondences} placed on the surface. Several algorithms generate a PDM provided with a set of shapes, such as \cite{shapeworks, mdl, spharm}. However, all these algorithms require an implicit surface representation like segmentations/meshes, which requires manual intervention and anatomy-specific expertise. Additionally, these algorithms require a pre-processing pipeline involving re-sampling, rigid alignment, and smoothing, which is expensive in terms of computation and human resources. 

PDM algorithm captures the shape of the anatomy, and the shape is devoid of location and alignment information. Hence, these algorithms utilize the concept of \emph{world} and \emph{local} coordinate systems \cite{some citation here}. The local coordinates are correspondences that lie on the surface of a given shape. The world coordinates apply a rigid transformation on the local coordinates and bring the correspondences to a coordinate system that factors-out rigid alignment and location information, and are utilized for subsequent shape analysis. 

Recent work presented in \cite{bhalodia2018deepssm, uncertain}, have proposed a deep-learning-based approach to circumvent the resource-heavy computation in PDM model generation. They train a PDM directly from the raw 3D volumes, which mitigates segmentation and pre-processing during inference on a new image and facilitates a fully end-to-end automatic pipeline for shape analysis. The models are geared towards statistical shape modeling and are trained to predict the world coordinates of the PDM. However, when predicted directly from a 3D image, the local coordinates of PDM also have utility. They can be used for anatomy segmentation or as a coarse estimation of the anatomical surface.

In this paper, we propose a novel extension of the network architecture in \cite{bhalodia2018deepssm} to predict both the local and world coordinates of the PDM jointly. We evaluate the proposed model's efficacy in shape modeling downstream applications as well as anatomy segmentation, and demonstrate it is comparable to baseline models trained individually on the world and local coordinates, respectively. 

%

% Here begins the introduction. Citing \cite{bhalodia2018deepssm}.

% Diagnostic images are useful tools for diagnosis in clinical applications.

% Anatomical forms provide clinically relevant information for diagnosis

% Point Distribution Model (PDM) is powerful in providing quantitative representations of shapes for statistical shape analysis

% Foreshadow here world and local coordinates, e.g., to perform shape statistics, global transformation (rotation and translation, and sometimes scale) should be factored out, resulting in a shape space where PDM is represented in global/world coordinates and configuration space where shapes are represented in local coordinates (particles that lie on the surface).

% Conventional preprocessing for PDM is expensive in terms of time and efforts

% DeepSSM directly obtains PDM from images, either original local or world (local with Procrustes) particles

% We previously used DeepSSM to predict world particles for analysis

% We would like to get local particles to benefit other tasks, e.g. object detection, finer segmentation, explainability

% Show how segmentation/statistical models can benefit from this
% Our local predictions is composed of world and transformation predictions
% For the statistical shape models:
% our model decouples the transformations thus it generalizes to realistic applications where images are not aligned
% For the segmentation:
% Our local prediction is segmentation regularized by shape prior  thus robust to noise/outliers
% Our transformation prediction provides a Region of Interest as the basis for finer segmentation

% We need to add here a discussion on relevant works.

% Procrustes in shape analysis builds ground truth transformations with high accuracy

% We force the network learn transformations by augmenting transformations in training data

% We devised a loss function to supervise on transformations

% Losses are relative so multiple tasks are balanced during learning

% A training strategy of 2 phases are used to deal with local minimums while getting the best fit of the network



==> related_works.tex <==
\section{Related Works}
\label{sec:rw}
\TODO{Combined the intro and related works into one, we do not have much space.}
% Population shape analysis finds applications in different biomedical domains such as pathology characterization \cite{neuro, cardio}, growth modeling \cite{growth} and implant design \cite{implant}. The shape can be represented in variety of different ways, explicitly via meshes/point correspondences \cite{PDM} or, implicitly via segmentation/transformation fields \cite{transforms}. Particle Distribution Models (PDMs) places a dense set of correspondences on the anatomical surface, and these algorithms work via non-linear optimization \cite{Shpaeworks, MDL} or using pairwise comparison approach \cite{spharm}. 
% Transformations or deformations fields between images/volumes can also be used for representing the shape. 




